Efficient Primal-Dual Algorithms for Large-Scale Multiclass Classification

We develop efficient algorithms to train $\ell_1$-regularized linear classifiers with large dimensionality $d$ of the feature space, number of classes $k$, and sample size $n$. Our focus is on a special class of losses that includes, in particular, the multiclass hinge and logistic losses. Our approach combines several ideas: (i) passing to the equivalent saddle-point problem with a quasi-bilinear objective; (ii) applying stochastic mirror descent with a proper choice of geometry which guarantees a favorable accuracy bound; (iii) devising non-uniform sampling schemes to approximate the matrix products. In particular, for the multiclass hinge loss we propose a \textit{sublinear} algorithm with iterations performed in $O(d+n+k)$ arithmetic operations.

==> alg-main-old.tex <==
\begin{algorithmic}[1]
\REQUIRE \mbox{$X \in \R^{n \times d}$,~$y \in [k]^{\otimes n}$,~$\lambda$,~$R_*$, $T \geqs 1$,~$\{\gamma_t\}_{t = 0}^{T-1}$}
%\vspace{-0.3cm}
%\item[\#] {\em Initialization}
\STATE Obtain~$Y \in \Delta_k^{\otimes n}$ from the label vector~$y$
\STATE $\wh X = [X,-X]$
%\STATE $Y = \zeros_{n \times k}$
%\FOR{$j = 1$ \TO $n$}
%\STATE $Y(j,y_j) = 1$
%\ENDFOR
\STATE $\alpha^0 = \ind_{2d}$; \; $\wt U^0 = \frac{R_{*}}{2dk} \cdot \ind_{2d \times k}$ 
\STATE $\beta^0 = \ind_{n}$;  \;\; $\wt V^0 = \frac{1}{k} \cdot \ind_{n \times k}$ %\COMMENT{Uniform distributions}
\FOR{$\imath=1$ \TO $2d$}
\STATE $\sigma({\imath}) = \|\wh{X}(:,\imath)\|_2$; \;\;\, $\pi^0(\imath) = \|\wt{U}^0(\imath,:)\|_1 \equiv R_*$
\ENDFOR
\FOR{$\jmath=1$ \TO $n$}
\STATE $\tau(\jmath) = \|\wh{X}(\jmath,:)\|_\infty$; \;  $\rho^0(\jmath) = \|\wt{V}^0(\jmath,:) - Y(\jmath,:)\|_1$ % $\rho^0(\jmath) = \|\wt{V}^0(\jmath,:) \cdot \beta^0(\jmath) - Y(\jmath,:)\|_1$
\ENDFOR
\item[\#] {\em Initialize machinery to track the cumulative sums}
\STATE $\Usum^0  = 0_{2d\times k}$; \;\, $\Vsum^0 = 0_{n\times k}$ \COMMENT{Cumulative sums}
\STATE $\Acur^0 = \zeros_{2d}$; \; $\Bcur^0 = 0_{n}$; \; $\Aprev^0 = 0_{2d\times k}$; \; $\Bprev^0 = 0_{n\times k}$; 
%\STATE 
%$\Aprev^0 = 0_{2d\times k}$; \; $\Bprev^0 = 0_{n\times k}$
%\item[\#] {\em Iterate stochastic mirror descent with full sampling}
\FOR[\eqref{StochasticUpdates} iterations]{$t=0$ \TO $T-1$}
%\item[\#] {\em Primal updates}
\item[\#] {\em Choose a random example and a class, cf.~\eqref{eq:optimal-probabilities-full}} 
%\item[\#] {\em $\circ$ is the elementwise product} 
\STATE Draw~$j^t \sim \tau \circ \rho^t$
\STATE Draw~$l^t \sim | \wt V^{t}(\jt,:) \cdot \beta^t(j^t)   -Y(\jt,:)|$ 
\STATE $[\Usum^{t+1}, \Aprev^{t+1}, \Acur^{t+1}]$ \\ \quad $\gets \textsc {TrackSumPrimal}(\wt U^t, \Usum^t, \Aprev^t, A^t,\alpha^t,l^t)$
\item[\#] {\em The only non-zero column of~$\eta_{V^t,Y}$, cf.~\eqref{eq:full-sampling}:}
\STATE ${\eta}^{t} = \wh{X}(j^t,:) \cdot \frac{\sum_{\jmath=1}^n \tau(\jmath) \cdot \rho^t(\jmath)\cdot\sgn[\beta^t_{\jmath} \cdot V(\jmath,l^t)-Y(\jmath,l^t)]}{\tau({j^t})}$
\label{alg:line-eta}
\STATE $[\wt{U}^{t+1}, \alpha^{t+1}, \pi^{t+1}] $ \\ \quad $\gets \textsc {UpdatePrimal}(\wt U^t, \alpha^t, \pi^t, \eta^t, l^t, \gamma_t, \lambda, R_*)$ %using \eqref{UpdatesAlphaU}
%\item[\#] {\em Track primal averages}
%\FOR{$i=1$ \TO $2d$}
%\STATE Update $\Acur^{t+1}_i, (\Aprev^{t+1})_i, (\Usum^{t+1})_i$ using \eqref{UpdatesUSum}
%\ENDFOR
%\item[\#] {\em Dual updates}
\item[\#] {\em Choose a random feature and a class, cf.~\eqref{eq:optimal-probabilities-full}}
\STATE Draw $\it  \sim \sigma \circ \pi^t$ 
\STATE Draw $\ell^t \sim \wt U^t(\it,:)$
\STATE $[\Vsum^{t+1}, \Bprev^{t+1}, \Bcur^{t+1}]$ \\ \quad $\gets \textsc {TrackSumDual}(\wt V^t, \Vsum^t, \Bprev^t, B^t,\beta^t,\ell^t,y)$
\item[\#] {\em The only non-zero column of~$\xi_{U^t}$, cf.~\eqref{eq:full-sampling}:}
\STATE $\xi^{t} =  \wh{X}(:,i^t) \cdot \frac{\sum_{\imath=1}^{2d}  \sigma(\imath)^{\vphantom{t}} \cdot \pi^t(\imath)}{\sigma(i^t)}$
\label{alg:line-xi}
\STATE $[\wt{V}^{t+1}, \beta^{t+1}, \rho^{t+1}]$ \\ \quad  $\gets \textsc {UpdateDual}(\wt V^t, Y, \beta^t, \rho^t, \xi^t, \ell^t, y, \gamma_t)$ %using \eqref{UpdatesAlphaU}
%\STATE Evaluate~$(s^{V})^{t}\in \R^n$ and~$\chi^{t}\in \R^n$~using~\eqref{xiUpdates}
%\item[\#] {\em Track dual averages}
%\FOR{$j=1$ \TO $n$}
%\STATE Update $\Bcur^{t+1}_i, (\Bprev^{t+1})_i,(\Vsum^{t+1})_i$ using~\eqref{UpdatesVSum}
%\ENDFOR
\ENDFOR
\FOR{$l = 1$ \TO $k$}
\STATE $\Usum^T(:,l) = \Usum^{T}(:,l) + \wt{U}^{T}(:,l) \circ (\alpha^T + \Acur^T - \Aprev^{T}(:,l))$
\label{alg:line-post-prim}
\STATE $\Vsum^T(:,l) = \Vsum^{T}(:,l) + \wt{V}^{T}(:,l) \circ (\beta^T + \Bcur^T - \Bprev^{T}(:,l))$
\label{alg:line-post-dual}
\ENDFOR
\ENSURE $\bar{U}^T = \frac{1}{T}\Usum^T,$~$\bar{V}^T = \frac{1}{T} \Vsum^T$
\end{algorithmic}
